StudioGAN: A Taxonomy and Benchmark of GANs for Image Synthesis

Generative Adversarial Network (GAN) is one of the state-of-the-art generative models for realistic image synthesis. While training and evaluating GAN becomes increasingly important, the current GAN research ecosystem does not provide reliable benchmarks for which the evaluation is conducted consistently and fairly. Furthermore, because there are few validated GAN implementations, researchers devote considerable time to reproducing baselines. We study the taxonomy of GAN approaches and present a new open-source library named StudioGAN. StudioGAN supports 7 GAN architectures, 9 conditioning methods, 4 adversarial losses, 12 regularization modules, 3 differentiable augmentations, 7 evaluation metrics, and 5 evaluation backbones. With our training and evaluation protocol, we present a large-scale benchmark using various datasets (CIFAR10, ImageNet, AFHQv2, FFHQ, and Baby/Papa/Granpa-ImageNet) and 3 different evaluation backbones (InceptionV3, SwAV, and Swin Transformer). Unlike other benchmarks used in the GAN community, we train representative GANs, including BigGAN and StyleGAN series in a unified training pipeline and quantify generation performance with 7 evaluation metrics. The benchmark evaluates other cutting-edge generative models (e.g., StyleGAN-XL, ADM, MaskGIT, and RQ-Transformer). StudioGAN provides GAN implementations, training, and evaluation scripts with the pre-trained weights. StudioGAN is available at https://github.com/POSTECH-CVLab/PyTorch-StudioGAN.

==> Main_Material/Tables/post_processing_temp.tex <==
\begin{table}[!htp]
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{clccc}
\cmidrule[1.0pt]{2-5}
& \multirow{1}*[0.0ex]{\textsc{Resizer}~$\circled2$ \& $\circled3$} & \multirow{1}*[0.0ex]{\textsc{IS}~$\uparrow$} & \multirow{1}*[0.0ex]{\textsc{Top-1 acc.}~$\uparrow$} & \multirow{1}*[0.0ex]{\textsc{Top-5 acc.}~$\uparrow$} \\\cmidrule[1.0pt]{2-5}
\parbox[t]{3mm}{\multirow{13}{*}{\rotatebox[origin=c]{90}{\text{InceptionV3}~\cite{Szegedy2016RethinkingTI}}}} 
\parbox[t]{0.5mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\text{128}}}}
& \textsc{Nearest}&  167.06  &  67.88   & 88.07  \\
& \cellcolor{gray!20}\textbf{\textsc{Bilinear}} &  \cellcolor{gray!20}\textbf{182.57}  &  \cellcolor{gray!20}\textbf{72.03}   & \cellcolor{gray!20}\textbf{90.09} \\
& \textsc{Bicubic}~\cite{Keys1981CubicCI} & 178.45 & 71.84 & 89.80\\ 
& \textsc{Lanczos}~\cite{Turkowski1990FiltersFC} & 173.79 & 71.42 & 89.53 \\ 
\cmidrule[1.0pt]{2-5}
\parbox[t]{3mm}{\multirow{13}{*}{\rotatebox[origin=c]{90}{}}} 
\parbox[t]{0.5mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\text{256}}}}
& \textsc{Nearest}& 260.17 & 77.65   & 93.98 \\
& \cellcolor{gray!20}\textbf{\textsc{Bilinear}} & \cellcolor{gray!20}\textbf{259.55} &  \cellcolor{gray!20}\textbf{78.11}  & \cellcolor{gray!20}\textbf{94.08} \\
& \textsc{Bicubic}~\cite{Keys1981CubicCI} & 259.99 & 78.26 & 94.16 \\ 
& \textsc{Lanczos}~\cite{Turkowski1990FiltersFC} & 259.31 & 78.27 & 94.13 \\ 
\cmidrule[1.0pt]{2-5}
\parbox[t]{3mm}{\multirow{13}{*}{\rotatebox[origin=c]{90}{}}} 
\parbox[t]{0.5mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\text{512}}}}
& \textsc{Nearest}& 262.30 & 77.89 & 94.00\\
& \cellcolor{gray!20}\textbf{\textsc{Bilinear}} & \cellcolor{gray!20}\textbf{265.22} & \cellcolor{gray!20} \textbf{78.48} & \cellcolor{gray!20}\textbf{94.30}\\
& \textsc{Bicubic}~\cite{Keys1981CubicCI} & 265.14 & 78.44 & 94.30 \\ 
& \textsc{Lanczos}~\cite{Turkowski1990FiltersFC} & 264.32 & 78.41 & 94.26 \\ 
\cmidrule[1.0pt]{2-5}
\morecmidrules
\cmidrule[1.0pt]{2-5}
\parbox[t]{3mm}{\multirow{13}{*}{\rotatebox[origin=c]{90}{\text{SwAV}~\cite{Caron2020UnsupervisedLO}}}}
\parbox[t]{0.5mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\text{128}}}}
& \textsc{Nearest}&  153.46  &  59.71   & 82.80  \\
& \cellcolor{gray!20}\textbf{\textsc{Bilinear}} &  \cellcolor{gray!20}\textbf{276.67}  &  \cellcolor{gray!20}\textbf{69.78}   & \cellcolor{gray!20}\textbf{89.46} \\
& \textsc{Bicubic}~\cite{Keys1981CubicCI} & 273.76 & 69.26 & 88.99\\ 
& \textsc{Lanczos}~\cite{Turkowski1990FiltersFC} & 254.81 & 68.36 & 88.37 \\ 
\cmidrule[1.0pt]{2-5}
\parbox[t]{3mm}{\multirow{13}{*}{\rotatebox[origin=c]{90}{}}} 
\parbox[t]{0.5mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\text{256}}}}
& \textsc{Nearest}& 299.90 &  72.79   & 91.15 \\
& \cellcolor{gray!20}\textbf{\textsc{Bilinear}} & \cellcolor{gray!20}\textbf{327.90} & \cellcolor{gray!20}\textbf{74.39}  & \cellcolor{gray!20}\textbf{92.06} \\
& \textsc{Bicubic}~\cite{Keys1981CubicCI} & 321.78 & 74.04 & 91.85 \\ 
& \textsc{Lanczos}~\cite{Turkowski1990FiltersFC} & 316.78 & 73.68 & 91.64 \\ 
\cmidrule[1.0pt]{2-5}
\parbox[t]{3mm}{\multirow{13}{*}{\rotatebox[origin=c]{90}{}}} 
\parbox[t]{0.5mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\text{512}}}}
& \textsc{Nearest}& 302.56 & 72.57 & 91.22\\
& \cellcolor{gray!20}\textbf{\textsc{Bilinear}} & \cellcolor{gray!20}\textbf{341.60} & \cellcolor{gray!20} \textbf{74.66} & \cellcolor{gray!20}\textbf{92.25}\\
& \textsc{Bicubic}~\cite{Keys1981CubicCI} & 334.83 & 74.34 & 92.04 \\ 
& \textsc{Lanczos}~\cite{Turkowski1990FiltersFC} & 326.64 & 73.99 & 91.78 \\ 
\cmidrule[1.0pt]{2-5}
\morecmidrules
\cmidrule[1.0pt]{2-5}
\parbox[t]{3mm}{\multirow{13}{*}{\rotatebox[origin=c]{90}{\text{DINO}~\cite{caron2021emerging}}}}
\parbox[t]{0.5mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\text{128}}}}
& \textsc{Nearest}&  376.96  &  73.82   & 91.47  \\
& \cellcolor{gray!20}\textbf{\textsc{Bilinear}} &  \cellcolor{gray!20}\textbf{460.49}   &  \cellcolor{gray!20}\textbf{78.47}   & \cellcolor{gray!20}\textbf{94.14} \\
& \textsc{Bicubic}~\cite{Keys1981CubicCI} & 452.35 & 78.07 & 93.94\\ 
& \textsc{Lanczos}~\cite{Turkowski1990FiltersFC} & 438.38 & 77.34 & 93.57 \\ 
\cmidrule[1.0pt]{2-5}
\parbox[t]{3mm}{\multirow{13}{*}{\rotatebox[origin=c]{90}{}}} 
\parbox[t]{0.5mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\text{256}}}}
& \textsc{Nearest}& 474.69 &  78.92   & 94.39 \\
& \cellcolor{gray!20}\textbf{\textsc{Bilinear}} & \cellcolor{gray!20}\textbf{485.45} & \cellcolor{gray!20}\textbf{79.70}  & \cellcolor{gray!20}\textbf{94.72} \\
& \textsc{Bicubic}~\cite{Keys1981CubicCI} & 484.10 & 79.62 & 94.64 \\ 
& \textsc{Lanczos}~\cite{Turkowski1990FiltersFC} & 480.31 & 79.39 & 94.51 \\ 
\cmidrule[1.0pt]{2-5}
\parbox[t]{3mm}{\multirow{13}{*}{\rotatebox[origin=c]{90}{}}} 
\parbox[t]{0.5mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\text{512}}}}
& \textsc{Nearest}& 464.84 & 78.39 & 94.11\\
& \cellcolor{gray!20}\textbf{\textsc{Bilinear}} & \cellcolor{gray!20}\textbf{487.74} & \cellcolor{gray!20}\textbf{79.79} & \cellcolor{gray!20}\textbf{94.79}\\
& \textsc{Bicubic}~\cite{Keys1981CubicCI} & 486.49 & 79.67 & 94.71 \\ 
& \textsc{Lanczos}~\cite{Turkowski1990FiltersFC} & 482.97 & 79.50 & 94.63 \\ 
\cmidrule[1.0pt]{2-5}
\end{tabular}}
\end{table}

==> Main_Material/Tables/pre_processing.tex <==
\begin{table}[!htp]
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{clcccc}
\cmidrule[1.0pt]{2-6}
& \multirow{2}*[0.0ex]{\textsc{Resizer} $\circled1$} & \multirow{2}*[0.0ex]{\textsc{IS}~$\uparrow$} & \multirow{2}*[0.0ex]{\textsc{FID}~$\downarrow$} & \multirow{2}*[0.0ex]{\textsc{Top-1 acc.}~$\uparrow$} & \multirow{2}*[0.0ex]{\textsc{Top-5 acc.}~$\uparrow$} \\
\parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{\text{ImageNet}~\cite{Brock2019LargeSG}}}}
&  & & & & \\\cmidrule[1.0pt]{2-6}
& \textsc{Nearest} &  TBD  &  TBD  &  TBD  &  TBD.  \\
& \textsc{Bilinear} &  TBD  &  TBD  &  TBD  &  TBD.  \\
& \textsc{Bicubic}~\cite{Keys1981CubicCI}   & TBD  &  TBD  &  TBD  &  TBD.  \\
& \textsc{Lanczos}~\cite{Turkowski1990FiltersFC}  & TBD  &  TBD  &  TBD  &  TBD.  \\
\cmidrule[1.0pt]{2-6}
\end{tabular}}
\label{table:pre_processing}
\end{table}

==> Main_Material/Tables/shortcut_temp.tex <==
\begin{table}[!htp]
\resizebox{0.46\textwidth}{!}{
\begin{tabular}{clccc}
\cmidrule[1.0pt]{2-5}
\parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{\text{InceptionV3}}}}
\parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{\text{-TensorFlow}}}}
& \textsc{Resizer} \circled{5} & \textsc{\{I, S, T\}S}~$\uparrow$ &   \textsc{Top-1}~$\uparrow$    &  \textsc{Top-5}~$\uparrow$   \\
\cmidrule[1.0pt]{2-5}
& \textsc{Nearest} &  256.82  &   77.35  &  93.66  \\
& \cellcolor{gray!20}\textbf{\textsc{bilinear}} &  \cellcolor{gray!20}\textbf{266.00}  &   \cellcolor{gray!20}\textbf{78.46} &  \cellcolor{gray!20}94.27  \\
& \textsc{Bicubic}~\cite{Keys1981CubicCI} &  265.92  &   78.45 &  \textbf{94.31}  \\
& \textsc{Lanczos}~\cite{Turkowski1990FiltersFC} &  264.79  &   78.43  &  94.27  \\
\cmidrule[1.0pt]{2-5}
\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\text{SwAV}}}}
\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\text{-PyTorch}}}}
& \textsc{Nearest} &  275.67  &   71.11  &  90.55  \\
& \cellcolor{gray!20}\textbf{\textsc{bilinear}} &  \cellcolor{gray!20}\textbf{341.69}  &   \cellcolor{gray!20}\textbf{74.67}  &  \cellcolor{gray!20}\textbf{92.23}  \\
& \textsc{Bicubic}~\cite{Keys1981CubicCI} &  335.79  &   74.40  &  92.09  \\
& \textsc{Lanczos}~\cite{Turkowski1990FiltersFC} &  327.70  &  74.03 &  91.85  \\
\cmidrule[1.0pt]{2-5}
\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\text{Swin-T}}}}
\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\text{-PyTorch}}}}
& \textsc{Nearest} &  205.65  & 84.05  &  97.15 \\
& \textsc{bilinear} &  202.57  &   84.76  & 97.41  \\
&  \cellcolor{gray!20}\textbf{\textsc{Bicubic}}~\cite{Keys1981CubicCI} &  \cellcolor{gray!20}\textbf{214.77} &  \cellcolor{gray!20}\textbf{85.22} &  \cellcolor{gray!20}\textbf{97.51}  \\
& \textsc{Lanczos}~\cite{Turkowski1990FiltersFC} &  214.56  & 85.09  &  97.46  \\
\cmidrule[1.0pt]{2-5}
\end{tabular}}
\label{table:shortcut}
\end{table}

==> Main_Material/Tables/temp.tex <==
\begin{table*}
        \centering
        \captionof{table}{\label{tab:main_table}Performance on standard benchmarks in accuracy, FLOPs, per-pair inference time, and memory footprint. Subscripts denote backbone networks. Some results are from ~\cite{jeon2018parn,kim2018recurrent, li2020correspondence,liu2020semantic,min2019hyperpixel,min2020dhpf,cho2021semantic}. Numbers in bold indicate the best performance and underlined ones are the second best. Models with an asterisk ($^{*}$) are retrained using keypoint annotations (strong supervision) from~\cite{li2020correspondence}. The first column shows supervisory signals used in training: image-level labels (I), and keypoint matches (K). The second column indicates the use of multi-level backbone features. FLOPs, per-pair inference time and memory footprints are measured on our machine with an Intel i7-7820X and an NVIDIA Titan-XP. The results in last two sections show our results with CP-CHM (top) and CHM (bottom) layers.
        }
        \scalebox{0.9}{
        \begin{tabular}{ccclccccccccccc}
                \toprule
                \multirow{3}{*}{Sup.} & \multirow{3}{*}{\shortstack{data\\aug.}} & \multirow{3}{*}{\shortstack{uses\\multi\\layer?}} & \multirow{3}{*}{Methods} & \multicolumn{2}{c}{SPair-71k} & \multicolumn{2}{c}{PF-PASCAL} & \multicolumn{3}{c}{PF-WILLOW} & \multirow{3}{*}{\shortstack{uses\\nD conv?}} & \multirow{3}{*}{\shortstack{FLOPs\\(G)}} & \multirow{3}{*}{\shortstack{time\\({\em ms})}} & \multirow{3}{*}{\shortstack{memory\\(GB)}} \\
                
                 & & & & \multicolumn{2}{c}{PCK @ $\alpha_{\text{bbox}}$} & \multicolumn{2}{c}{PCK @ $\alpha_{\text{img}}$} & \multicolumn{2}{c}{PCK @ $\alpha_{\text{bbox}}$} & PCK @ $\alpha_{\text{bbox-kp}}$ & &  &  & \\ 
                 
                 & & & & 0.1 (F) & 0.1 (T) & 0.05 & 0.1 & 0.05 & 0.1 & 0.1 & & & & \\
                 
                 \midrule
                 
                 \multirow{4}{*}{\shortstack{I}} & \xmark & \xmark & NC-Net$_\textrm{res101}$~\cite{rocco2018neighbourhood} & 20.1 & 26.4 & {54.3} & 78.9 & - & - & 67.0 & 4D & 44.9 & 222 & \underline{1.2} \\
                 
                 & \xmark & \xmark & DCC-Net$_\textrm{res101}$~\cite{huang2019dynamic}  & - & 26.7 & {55.6} & {82.3} & - & - & 73.8 & 4D & 47.1 & 567 & 2.7 \\
                 
                 & \xmark & \cmark & DHPF$_\textrm{res101}$~\cite{min2020dhpf}  & 27.7 & 28.5 & {56.1} & {82.1} & 50.2 & \textbf{80.2} & 74.1 & \xmark & \textbf{2.0} & {58} & 1.6 \\
                 
                 & \xmark & \xmark & PMD$_\textrm{res101}$~\cite{li2021pmdnet} &  26.5 & - & - & 81.2 & - & - & 74.7 & \xmark & - & - & - \\
                 
                 \midrule
                 
                 \multirow{15}{*}{\shortstack{K}} 
                 & \xmark & \xmark & UCN$_\textrm{res101}$~\cite{choy2016universal}          & - & 17.7 & - & 75.1 & - & - & - & \xmark & - & - & - \\
                 
                 & \xmark & \cmark & HPF$_{\textrm{res101}}$~\cite{min2019hyperpixel}      &  28.2 & - & 60.1 & 84.8 & - & - & 74.4 & \xmark & - & 63 & - \\
                 
                 
                 & \xmark & \cmark & SCOT$_\textrm{res101}$~\cite{liu2020semantic} & 35.6 & - & 63.1 & 85.4 & - & - & \textbf{76.0} & \xmark & {6.2} & 151 & 4.6 \\
                 
                 
                 
                 & \xmark & \xmark & SCNet$_{\textrm{res101}}$~\cite{han2017scnet}           & - & - & 36.2 & 72.2 & 38.6 & 70.4 & - & \xmark & - & $>$1000 & - \\
                 
                 & \xmark & \cmark & DHPF$_{\textrm{res101}}$~\cite{min2020dhpf}           & {37.3} & 27.4  & {75.7} & {90.7} & 49.5 & 77.6 & 71.0 & \xmark & \textbf{2.0} & {58} & 1.6 \\
                 
                 & \xmark & \xmark & NC-Net$^\textrm{\textbf{*}}_\textrm{res101}$~\cite{rocco2018neighbourhood} & - & - & - & 81.9 & - & - & - & 4D & 44.9 & 222 & \underline{1.2} \\
                 
                 & \xmark & \xmark & DCC-Net$^\textrm{\textbf{*}}_\textrm{res101}$~\cite{huang2019dynamic} &  - & - & - & 83.7 & - & -  & - & 4D & 47.1 & 567 & 2.7 \\
                 
                 & \xmark & \xmark & ANC-Net$_\textrm{res101}$~\cite{li2020correspondence} &  - & \underline{28.7} & - & 86.1 & - & - & - & 4D & 44.9 & 216 & \textbf{0.9} \\
                 
                 & \xmark & \xmark & PMD$_\textrm{res101}$~\cite{li2021pmdnet} &  37.4 & - & - & 90.7 & - & - & \underline{75.6} & \xmark & - & - & - \\
                 
                 & \xmark & \cmark & PMNC$_\textrm{res101}$~\cite{lee2021patchmatchnc} &  50.4 & - & \underline{82.4} & 90.6 & - & - & - & 4D & - & 960 & 2.6 \\
                 
                 & \cmark & \cmark & CATs$_\textrm{res101}$~\cite{cho2021semantic}   & 49.9 & - & 75.4 & \underline{92.6} & 50.3 & 79.2 & 69.0 & \xmark & - & \underline{35} & 1.6 \\
                 
                 & \xmark & \cmark & CATs$_\textrm{res101}$~\cite{cho2021semantic}   & 43.5 & - & - & - & - & - & - & \xmark & - & \underline{35} & 1.6 \\
                 
                 \cline{2-15} \\[-1.8ex]
                 
                 
                 
                 & \cmark & \cmark & CHMNet$_\textrm{res101}^{\text{CP-CHM}}$ (ours)   & \textbf{51.3} & 26.1 & \textbf{83.1} & \textbf{92.9} & \textbf{53.8} & {79.3} & 69.3 & 3D+3D & 7.2 & {43} & 1.8 \\
                
                 & \xmark & \cmark & CHMNet$_\textrm{res101}^{\text{CP-CHM}}$ (ours)   & {47.0} & 27.6 & 81.2 & 91.5 &  {51.9} & 77.0 & 67.3 & 3D+3D & 7.2 & 41 & 1.8 \\
                 
                 & \xmark & \xmark & CHMNet$_\textrm{res101}^{\text{CP-CHM}}$ (ours)   & 46.2 & 26.5 & 80.1 & 90.7 & 48.9 & 72.6 & 63.4 & 3D+3D & \underline{3.4} & \textbf{32} & 1.5 \\ 
                 \cline{2-15} \\[-1.8ex]
                 
                 & \cmark & \cmark & CHMNet$_\textrm{res101}$ (ours)   & \underline{51.1} & 26.8 & 80.8 & \textbf{92.9} & \textbf{53.8} & 79.0 & 69.6 & 6D & 21.2 & 62 & 1.8 \\
                 
                 
                 
                 & \xmark & \xmark & CHMNet$_\textrm{res101}$ (ours)   & {46.3} & \textbf{30.1} & {80.1} & {91.6} & \underline{52.7} & \underline{79.4} & 69.6 & 6D & 19.6 & 54 & 1.6 \\
                 
                 
                \bottomrule
        \end{tabular}
        }
\end{table*}

==> Main_Material/sota_generation.tex <==
\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.31\linewidth]{Main_Material/Figures/imagenet.pdf}
    \hspace{-0.20cm}
    \includegraphics[width=0.31\linewidth]{Main_Material/Figures/cub.pdf}
    \hspace{-0.30cm}
    \includegraphics[width=0.205\linewidth]{Main_Material/Figures/tiny_imagenet.pdf}
    \hspace{-0.25cm}
    \includegraphics[width=0.16\linewidth]{Main_Material/Figures/cifar.pdf}
    \caption{Generation results of SOTA GANs on CIFAR10, Baby-ImageNet, ImageNet, and AFHQv2.}
    \label{fig:sota_qualitative_images}
\end{figure*}

==> Sections/2_related_work.tex <==
\section{Generative Adversarial Network}
\label{sec:generatve_adversarial_network}

In 2014, Goodfellow~\etal~\cite{Goodfellow2014GenerativeAN} proposed a new framework for generative modeling on the basis of a two-player game. The framework named Generative Adversarial Network~(GAN) aims to estimate the distribution of an arbitrary dataset in high-dimensional space and consists of a generator and a discriminator network adversarial to each other. Specifically, the \emph{generator} $G: \mathcal{Z}\longrightarrow\mathcal{X}$ strives to map a latent variable $\rvz \sim p(\rvz)$ into a sample $G(\rvz)$ as if the sample is drawn from the real data distribution $p(\rvx)$. The \emph{discriminator} $D:\mathcal{X}\longrightarrow[0,1]$, on the other hand, tries to discriminate whether \minguk{a}the given sample comes from the real data distribution or from the generator, becoming the adversary to the generator. Mathematically, the generative and discriminative processes can be expressed as follows:
\begin{align*}
    \min_{G}\max_{D}~\mathbb{E}_{\rvx \sim {p(\rvx)}}[\log(D(\rvx))] + \mathbb{E}_{\rvz \sim {p(\rvz)}}[\log(1 - D(G(\rvz)))].
    \label{eq:eq1}\tag{1}
\end{align*}
Goodfellow~\etal~\cite{Goodfellow2014GenerativeAN} demonstrate that the adversarial training between the two networks converges to Nash equilibrium~\cite{Nash1951NONCOOPERATIVEG} under the two assumptions: (1) the two models have enough capacity, and (2) the discriminator is allowed to reach its optimum against the generator at each step. Under these conditions, implicit distribution of the generator $p_{G(\rvz)}(\rvx)$ converges to the true data distribution $p(\rvx)$, and generator becomes an efficient sampler for the true data distribution. 

On the theoretical foundation of Goodfellow~\etal's study~\cite{Goodfellow2014GenerativeAN}, GAN has evolved with sophisticated architectures, advanced adversarial losses, and regularizations for stable training. Representatively, the authors of f-GAN verify that some of GAN objectives can be interpreted using f-divergence metric. Arjovsky~\etal~\cite{Arjovsky2017WassersteinG} analyze the source of instability in the perspective of probability theory. Although many solutions were proposed to stabilize GAN dynamics, most researches before the advent of Miyato~\etal's work~\cite{Miyato2018SpectralNF}, failed to synthesize high-quality images on a complex dataset, such as ImageNet~\cite{Deng2009ImageNetAL}. Spectral normalized GAN~(SNGAN) proposed by Miyato~\etal~\cite{Miyato2018SpectralNF} is the first GAN that succeeds in generating ImageNet dataset using only a single pair of the generator and the discriminator network. Following this success, SAGAN~\cite{Zhang2019SelfAttentionGA}, BigGAN~\cite{Brock2019LargeSG}, and ReACGAN~\cite{kang2021rebooting} raise the standard of natural image synthesis. While the above GANs show reasonable generation results, generating realistic images that even human eyes cannot distinguish, remains a crucial problem. Karras~\etal improve the generation quality of GAN by introducing more inductive bias into GAN architecture. StyleGAN~\cite{karras2019style}, StyleGAN2~\cite{karras2020analyzing}, and StyleGAN3~\cite{karras2021alias} proposed by Karras~\etal successfully generate high-resolution realistic images on well-processed datasets such as FFHQ~\cite{karras2019style}, AFHQ~\cite{choi2020starganv2}, and AFHQv2~\cite{choi2020starganv2, karras2021alias}.

Recently, data-efficient training techniques tailored to GAN are attracting attention from the image generation community. Since discriminator's overfitting problem is widely known to ruin the adversarial training~\cite{Brock2019LargeSG}, most data-efficient training techniques concentrate on preventive methods for the overfitting phenomenon, which gets worse as the number of data becomes insufficient. Karras~\etal~\cite{Karras2020TrainingGA} suggests adaptive discriminator augmentation~(ADA) that controls the strength of differentiable augmentations according to the confidence of the discriminator. At the same time, Zhao~\etal~\cite{zhao2020differentiable} develop differentiable augmentations (DiffAug) for GAN training and demonstrate the effectiveness of DiffAug both in data-hungry and data-enough situations. Tseng~\etal~\cite{lecam2021} propose LeCam regularization based on LeCam-divergence and show that GAN with LeCam regularization improves image generation quality in data-hungry circumstance.
